Large Language Model (LLM) for Software Security: Code Analysis, Malware Analysis, Reverse Engineering

Large Language Models (LLMs) have recently emerged as powerful tools in cybersecurity, offering advanced capabilities in malware detection, generation, and real-time monitoring. Numerous studies have explored their application in cybersecurity, demonstrating their effectiveness in identifying novel malware variants, analyzing malicious code structures, and enhancing automated threat analysis. Several transformer-based architectures and LLM-driven models have been proposed to improve malware analysis, leveraging semantic and structural insights to recognize malicious intent more accurately. This study presents a comprehensive review of LLM-based approaches in malware code analysis, summarizing recent advancements, trends, and methodologies. We examine notable scholarly works to map the research landscape, identify key challenges, and highlight emerging innovations in LLM-driven cybersecurity. Additionally, we emphasize the role of static analysis in malware detection, introduce notable datasets and specialized LLM models, and discuss essential datasets supporting automated malware research. This study serves as a valuable resource for researchers and cybersecurity professionals, offering insights into LLM-powered malware detection and defence strategies while outlining future directions for strengthening cybersecurity resilience.

==> Archive/PEfilesTable.tex <==

\begin{table}[h]
    \centering
    \resizebox{\textwidth}{!}{ % Resizes the table to fit within text width
    \begin{tabular}{|l|l|l|}
        \hline
        \textbf{PE File Type} & \textbf{Extension} & \textbf{Description} \\
        \hline
        Dynamic Link Library & .dll & Shared library files containing code and data for multiple programs. \\
        \hline
        Audio Compression Manager & .acm & Driver files used for audio compression in Windows. \\
        \hline
        MPEG-4 Filter File & .ax & DirectShow filter files used for processing video and audio streams. \\
        \hline
        Control Panel Extension & .cpl & Special DLL files used to add new Control Panel functionalities. \\
        \hline
        Driver File & .drv & Kernel-mode driver files for hardware and software interactions. \\
        \hline
        Extensible Firmware Interface File & .efi & PE files used in UEFI firmware to boot operating systems. \\
        \hline
        Multilingual User Interface File & .mui & Language resource files for UI localization in Windows applications. \\
        \hline
        Multilingual User Interface Resource File & .mun & Windows 10/11 resource files similar to .mui, used for UI translations and system elements. \\
        \hline
        ActiveX Control File & .ocx & Object files containing UI components for Windows applications. \\
        \hline
        Screensaver File & .scr & Executable screensaver files, similar to .exe. \\
        \hline
        Device Driver File & .sys & Low-level system driver files used by Windows to control hardware. \\
        \hline
        Telephony Service Provider File & .tsp & Files used by Windows telephony services for voice and modem communication. \\
        \hline
        Windows Theme File & .msstyles & Files that define the visual style (theme) of Windows UI elements. \\
        \hline
        Program Executable File & .exe & Standard executable files for launching programs in Windows. \\
        \hline
        Font File & .fon & Legacy bitmap font files in PE format. \\
        \hline
        Net Assembly & .exe, .dll & PE files containing managed code for .NET applications. \\
        \hline
    \end{tabular}
    }
    \caption{Common Portable Executable (PE) File Types and Their Descriptions}
    \label{tab:pe_files}
\end{table}



